Splicing Hints into Reasoning Traces: Learning from Demonstrator Failures

Reinforcement learning with verifiable rewards improves mathematical reasoning when a final answer can be checked, but a correct answer does not certify the derivation behind it, and proof problems offer no answer to check. Replacing the check with a reasoning model as an in-loop verifier faces a fundamental obstacle: the policy must already produce occasional correct attempts for any reward to exist, which it may never do at olympiad level. We instead move verification and repair out of the training loop and into offline data generation with SPLICE, a workflow in which a second model, given only a reference solution, edits a reasoning model's traces as they are generated: it verifies progress, truncates a failed trace at its last verified step, and splices in an adaptively strengthened hint until progress resumes. The resulting dataset includes repaired examples whose sampled unaided trajectory failed, with failed continuations removed and progress repeatedly checked against the reference solution. A model finetuned on SPLICE traces outperforms the same model distilled from the reasoning model's unedited traces on AIME and, under a grading protocol validated against human grades, on olympiad proofs. The trained model's own traces show a corresponding behavioral signature: at difficult points it announces a branch in the style of the spliced hints and takes riskier steps, with predictive entropy rising there and just after, a pattern absent from the model trained on unedited traces.

==> sections/statements.tex <==
\subsection*{AI use statement}
The SPLICE workflow, its design, the data selection and the experiments
are the authors' own. Language models are the object of study: the
demonstrator, the tutor and the grading judges are all language models,
and the training data are generated by the workflow of
Section~\ref{sec:method}, which is the subject of the paper. Beyond
that, generative AI served as a writing and coding assistant: it edited
and rephrased text, critiqued drafts as a reviewer would, and helped with
analysis scripts and figures. All AI-assisted text and code were reviewed
by the authors, all citations were verified by the authors, and the
authors take full responsibility for the manuscript and artifacts.

\subsection*{Reproducibility statement}

Section~\ref{sec:method} specifies the SPLICE loop and its stages, with
the models behind each stage in Appendix~\ref{app:tutor-models}, the
constants in Appendix~\ref{app:constants}, the stage signatures in
Appendix~\ref{app:signatures}, the prompt of every stage in
Appendix~\ref{app:prompts}, and the input--output contract of each stage
in Appendix~\ref{app:contracts}; Section~\ref{sec:training-data}
describes the problem sources. Section~\ref{sec:datasets} defines the
five datasets and the evaluation protocol, including the grading
procedure and the treatment of unfinished attempts, with the judge
validation in Appendix~\ref{app:grading} and the finetuning recipe and
evaluation settings in Appendix~\ref{app:training}. Code, generation
records, and evaluation outputs will be released on acceptance.

